Unsupervised Label Refinement Improves Dataless Text Classification

Dataless text classification is capable of classifying documents into previously unseen labels by assigning a score to any document paired with a label description. While promising, it crucially relies on accurate descriptions of the label set for each downstream task. This reliance causes dataless classifiers to be highly sensitive to the choice of label descriptions and hinders the broader application of dataless classification in practice. In this paper, we ask the following question: how can we improve dataless text classification using the inputs of the downstream task dataset? Our primary solution is a clustering based approach. Given a dataless classifier, our approach refines its set of predictions using k-means clustering. We demonstrate the broad applicability of our approach by improving the performance of two widely used classifier architectures, one that encodes text-category pairs with two independent encoders and one with a single joint encoder. Experiments show that our approach consistently improves dataless classification across different datasets and makes the classifier more robust to the choice of label descriptions.

==> abstract.tex <==
\begin{abstract}
\zewei{TODO: finish the abstract and submit before Sep 1st. Pick a name for our proposed approach? Discuss the paper layout/sections. How should the main table look like? Maybe ensembling different label choices for each task as our best results? What other baselines to compare to? +-+Paper deadline Sep 10th, i.e., next Thursday. }

% In this paper, we show how weakly supervised text classification models can be improved by two simple tricks, self-training and k-means clustering. 
Dataless text classification aims to classify text into categories without any annotated training data from the task of interest. 
% Prior works \zewei{\cite{yin2019benchmarking}, \natcat} show that by leveraging text and category resources from a variety of domains, models can be built to perform text classifications on provided sets of categories. 
% Without direct access to labeled training data from downstream tasks, 
Dataless classifiers rely on accurate descriptions of the label set for each downstream task. 
However, this reliance causes dataless classifiers to be highly sensitive to the choice of label descriptions.
%The fragility of dataless classifiers caused by the choices of label descriptions 
This fragility hinders the wider application of dataless classification in practice. 
% The wide application of the seemingly promising dataless text classifiers is hindered by their . 
% It is a difficult task for the end users to pick an optimal choice of label names in practical usage. 
In this paper, we ask the following question: how can we improve dataless text classification using the inputs of the downstream task dataset? 
% commented out label descriptions here because it's assumed that label descriptions are used by dataless classifiers.
%in addition to the label descriptions? 
Our primary solution is a clustering based approach. 
%With the initial semantic representations or scores of both text and categories produced by the dataless text classifiers, 
\kevin{since we talk about single vs dual encoder below, i  simplified the text here}
Given a dataless classifier, our approach %iteratively 
refines its set of predictions %such representations or scores by 
using K-means clustering. 
% With K-means clustering, our approach consistently improve the classification accuracy. 
We show how to apply this approach 
%can be naturally combined with 
to a variety of classifier architectures %dataless text classifiers 
to improve their performance, including those that use 
%Our approach can work on variations of dataless classifiers where either 
a single encoder or two separate encoders %are involved 
to score text-category pairs. 
%with different scoring measures. 
Experiments show that our approach improves dataless classification consistently across architectures and datasets and shows robustness across choices of label descriptions. 
% After combining our clustering approach with a \roberta based zero-shot text classifier, the average performance gap between the zero-shot classifier and human beings is within 10 points, making zero-shot text classifications have more practical use. 

\end{abstract}

